(Almost) All of Entity Resolution

Whether the goal is to estimate the number of people that live in a congressional district, to estimate the number of individuals that have died in an armed conflict, or to disambiguate individual authors using bibliographic data, all these applications have a common theme - integrating information from multiple sources. Before such questions can be answered, databases must be cleaned and integrated in a systematic and accurate way, commonly known as record linkage, de-duplication, or entity resolution. In this article, we review motivational applications and seminal papers that have led to the growth of this area. Specifically, we review the foundational work that began in the 1940's and 50's that have led to modern probabilistic record linkage. We review clustering approaches to entity resolution, semi- and fully supervised methods, and canonicalization, which are being used throughout industry and academia in applications such as human rights, official statistics, medicine, citation networks, among others. Finally, we discuss current research topics of practical importance.

==> subfiles/acknowledgements.tex <==
\section*{Acknowledgements}

O. Binette was supported by the Natural Sciences and Engineering Research Council of Canada, by the Fonds de Recherche du Québec --- Nature et Technologies.  O. Binette and R. C. Steorts were supported by NSF Career Award 1652431 and the Alfred P. Sloan Foundation. The authors thank Ted Enamorado for providing comments that greatly improved this work.



==> subfiles/related.tex <==
\section{Related work}
\label{sec:related}
The related work spans three key areas: ER methodology, inference for 
Bayesian ER models, and distributed MCMC.

\paragraph{Entity resolution methodology.}
Matching pairs of tables was first addressed with a probabilistic approach 
by \cite{newcombe_automatic_1959}. 
\cite{fellegi_theory_1969} later formalized this approach within the 
framework of decision theory.   
Many extensions to the Fellegi-Sunter (FS) model have been proposed 
(for surveys, see~\citealp{winkler_overview_2006, winkler2014matching}), 
including a recent extension to multiple 
databases~\citep{sadinle_generalized_2013}.
However, the FS model has been criticized 
due to its lack of support for duplicates within databases; 
false independence assumptions; and its dependence on 
subjective thresholds~\citep{tancredi_hierarchical_2011}.
These limitations have prompted development of more sophisticated 
Bayesian generative models, including models for bipartite 
matching~\citep{copas_record_1990, belin_1995, larsen_2001, 
  tancredi_hierarchical_2011, gutman_bayesian_2013, 
  sadinle_bayesian_2017}, 
de-duplication~\citep{sadinle_detecting_2014, steorts_entity_2015, 
  steorts_bayesian_2016}
and matching across multiple databases~\citep{steorts_entity_2015, 
  steorts_bayesian_2016}.
All of these models operate on structured data, and 
most~\citep{copas_record_1990, belin_1995, larsen_2001, 
  tancredi_hierarchical_2011, gutman_bayesian_2013, 
  steorts_bayesian_2016} rely solely on binary attribute-level 
comparisons to inform matching. 
Recent models~\citep{steorts_entity_2015, 
  sadinle_detecting_2014, sadinle_bayesian_2017} additionally 
utilize attribute-level similarity scores. 

% Our work builds on the Bayesian generative models of \cite{steorts_entity_2015,steorts_bayesian_2016} where 
% ER was framed as a bipartite matching problem between records 
% and latent entities.
% \cite{steorts_bayesian_2016} developed a fully hierarchical 
% Bayesian model assuming categorical attributes, with a Dirichlet 
% prior over the latent attributes and a data distortion model. 
% More recently, \cite{steorts_entity_2015} introduced a model 
% called \blink\ which extends \cite{steorts_bayesian_2016} to 
% both categorical and noisy string attributes using an 
% empirically-motivated prior. 
% The authors illustrated on real and simulated data that \blink\
% outperformed supervised methods when the training data was 10 
% percent (or less) of the total data. 
% In addition, the first tight performance bounds were shown for 
% \blink\ in \cite{steorts_performance_2017}. 
% As already mentioned, \blink\ has several limitations including 
% poor scalability, lack of support for missing values and 
% no native inclusion of probabilistic blocking, which are just a few of the contributions 
% of this paper. 

Apart from these advances in Bayesian approaches to matching 
(largely undertaken in statistics), there have 
been an abundance of contributions due to the database 
and machine learning communities 
\citep[see surveys by][]{getoor_entity_2012, christen_data_2012}.
Their focus has typically been on rule-based 
approaches~\citep{fan_reasoning_2009, singh_generating_2017}, 
supervised learning approaches~\citep{mudgal_deep_2018}, 
hybrid human-machine approaches~\citep{wang_crowder:_2012, 
  gokhale_corleone:_2014}, 
and scalability~\citep{papadakis_comparative_2016}.
Broadly speaking, all of these approaches rely on either humans in-the-loop 
or large amounts of labelled training data, which is not generally the 
case in the Bayesian setting.
%The hybrid human-machine approaches are a recent trend, 
%which leverage crowdsourcing to verify uncertain 
%matches~\cite{wang_crowder:_2012} or to supply labels 
%for active learning~\cite{gokhale_corleone:_2014}.

%The database community has leveraged Bayesian inference for merging, 
%with~\citep{zhao_bayesian_2012, pasternack_latent_2013} regarded as 
%key references in an area known also as truth finding (see 
%surveys by~\cite{li_survey_2016, zheng_truth_2017}). 
%While both approaches are generative, unsupervised and scale effectively,
%they apply post-matching only. 
%By contrast, this paper examines a Bayesian model that
%jointly infers matching and merging, a combination which incurs significant 
%challenges to scalability.

\paragraph{Inference for Bayesian ER models.}
Most prior work on Bayesian generative models for ER
\citep[e.g.][]{tancredi_hierarchical_2011, gutman_bayesian_2013,
  steorts_entity_2015} has relied on Gibbs 
sampling for inference. 
Compared to other Markov chain Monte Carlo (MCMC) algorithms, 
Gibbs sampling is relatively easy to implement, however it may suffer 
from slow convergence and poor mixing owing to its highly local 
moves~\citep{liu_monte_2004}.

In the broader context of clustering models, the \emph{split-merge 
	algorithm}~\citep{jain_split-merge_2004} has been proposed 
as a more efficient alternative to Gibbs sampling.
It traverses the space of clusterings through proposals that 
split single clusters or merge pairs of clusters, 
and is thus less susceptible to becoming trapped in local modes.
\cite{steorts_bayesian_2016} applied this algorithm to an ER model 
similar to \blink.
However it remains unclear whether the split-merge algorithm is 
appropriate for ER problems, where the number of clusters is 
expected to grow almost linearly in the number of 
records~\cite{zanella_flexible_2016}.

%More recently, \cite{zanella_flexible_2016} proposed the 
%\emph{chaperones algorithm} for inference in microclustering 
%models.
%It is similar in spirit to the split-merge algorithm, 
%however it is based on restricted Gibbs sampling 
%rather than the Metropolis-Hastings framework.
%It ``focuses on cluster reassignments with higher 
%probabilities'' by maintaining a biased distribution 
%over the space of record pairs.
%However, its scalability is likely to be limited as a result.

In this work, we apply partially-collapsed Gibbs 
sampling \citep{dyk_partially_2008}, as we expect it 
will be more efficient for ER models than the aforementioned 
methods, while still yielding an improvement over regular Gibbs 
sampling.

\paragraph{Parallel\slash distributed MCMC.}
Recent literature has focused on using parallel and 
distributed computing to scale up MCMC algorithms, 
where applications have  included Bayesian topic 
models~\citep{newman_distributed_2009, smola_architecture_2010, 
  ahn_distributed_2014} 
and mixture models~\citep{williamson_parallel_2013, 
  chang_parallel_2013, lovell_clustercluster:_2013, 
  ge_distributed_2015}.
We review the application to mixture models, as they are 
conceptually similar to ER models.

Existing work has concentrated on Dirichlet process (DP) 
mixture models and Hierarchical DP mixture 
models.\footnote{DP mixture models are not suitable for ER 
	applications as the cluster sizes grow linearly in the 
	number of records~\citep{zanella_flexible_2016}.
}
The key to enabling distributed inference for these 
models is the realization that a DP mixture model can 
be reparameterized as a mixture of DPs.
Put simply, the reparameterized model induces a 
\emph{partitioning} of the clusters, such that clusters 
assigned to \emph{distinct partitions} are conditionally 
independent. 
As a result, variables within partitions can be updated in parallel.

\cite{williamson_parallel_2013} exploited this idea at the 
thread level to parallelize inference for a DP mixture model.
\cite{chang_parallel_2013} followed a similar approach, but 
included an additional level of parallelization within partitions 
using a parallelized version of the split-merge algorithm.
Others~\citep{lovell_clustercluster:_2013, ge_distributed_2015} 
have developed distributed implementations in the Map-Reduce 
framework. 
While we do not consider DP mixture models in our work, 
we do borrow the reparameterization idea, albeit with a 
more flexible partition specification which helps with 
load balancing.

%\myparagraph{Paper organization.}
%The remainder of this paper proceeds as follows. 
%Related work is summarized next. 
%Section~\ref{sec:problem} describes the end-to-end Bayesian ER formulation for structured data.
%Section~\ref{sec:model} then (i) provides the details of the notation and model for Bayesian ER---\blink---and (ii) our proposed scalable formulation---\dblink. We specify how to partition entities in Section~\ref{sec:partition-fn} and how to perform inference efficiently in Sections~\ref{sec:inference} and~\ref{sec:tricks}. Section~\ref{sec:experiments} provides our comprehensive experimental evaluation.
